Uncertainty Informed Optimal Resource Allocation with Gaussian Process based Bayesian Inference

We focus on the problem of uncertainty informed allocation of medical resources (vaccines) to heterogeneous populations for managing epidemic spread. We tackle two related questions: (1) For a compartmental ordinary differential equation (ODE) model of epidemic spread, how can we estimate and integrate parameter uncertainty into resource allocation decisions? (2) How can we computationally handle both nonlinear ODE constraints and parameter uncertainties for a generic stochastic optimization problem for resource allocation? To the best of our knowledge current literature does not fully resolve these questions. Here, we develop a data-driven approach to represent parameter uncertainty accurately and tractably in a novel stochastic optimization problem formulation. We first generate a tractable scenario set by estimating the distribution on ODE model parameters using Bayesian inference with Gaussian processes. Next, we develop a parallelized solution algorithm that accounts for scenario-dependent nonlinear ODE constraints. Our scenario-set generation procedure and solution approach are flexible in that they can handle any compartmental epidemiological ODE model. Our computational experiments on two different non-linear ODE models (SEIR and SEPIHR) indicate that accounting for uncertainty in key epidemiological parameters can improve the efficacy of time-critical allocation decisions by 4-8%. This improvement can be attributed to data-driven and optimal (strategic) nature of vaccine allocations, especially in the early stages of the epidemic when the allocation strategy can crucially impact the long-term trajectory of the disease.

==> Bayesian_Inference_with_gamma.tex <==
%\vspace{-0.3cm}
\section{Bayesian Parameter Estimation}\label{sec: param_estimation_bayesian}
\vspace{-0.3cm}
%To solve the problem of incorporating \emph{uncertainty} in our estimates of the model parameters as well as in predicting new cases (in future) using an ODE system (SEIR model), we now  discuss Bayesian inference of model parameters. In particular, we aim to use Bayesian inference methods from literature \cite{calderhead} to estimate the \emph{joint-distribution} over model parameters from data instead of simply using point-estimates from NLLS. 

Bayesian inference for estimating ODE parameters has been studied in literature \cite{ramsay}, however in the absence of closed form posterior and
%large sample complexity associated 
the requirement of solving the ODE system in each sampling iteration  makes inference intractable. To overcome this limitation, \cite{calderhead} proposed the use of Gaussian Processes (GPs) to model the evolution of a state over time while exploiting the fact that derivative of a Gaussian process is also a Gaussian process. This significantly helps in achieving tractability and allows Bayesian inference to be computationally feasible. Following \cite{calderhead}, numerous other related works like \cite{dondelinger, barber, controversy, niu, nico, fgpgm, odin} have been proposed which also employ the use of GPs to efficiently estimate the posterior distribution on the parameters of a non-linear ODE system (for eg: SEIR model). We discuss some of these works useful to our problem next.

\iffalse
\SetVertexStyle[TextFont= \Large]
\begin{figure}[ht]
%\vspace{-0.25cm}
\centering
\begin{tikzpicture}
\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=2, y=0 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=0, y=0 ]{theta}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=4, y=0]{x}
\Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=2, y=2 ]{gamma}
\Edge[Direct=true,color= black, lw =1pt](theta)(x_dot)
\Edge[Direct=true,color= black,lw =1pt](gamma)(x_dot)
\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
\end{tikzpicture}
  %\vspace{-0.2cm}
    \caption{ODE model} \label{fig:graph_color}
    %\vspace{-0.15cm}
\end{figure}

\SetVertexStyle[TextFont= \Large]
\begin{figure}[ht]
%\vspace{-0.25cm}
\centering
\begin{tikzpicture}
\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=0, y=2 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=2, y=2]{x}
\Vertex[ size= 0.8,opacity =0, label = $\bm{y}$,             x=4, y=2 ]{y}
\Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=2, y=0 ]{phi}
\Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=4, y=0 ]{sigma}
\Edge[Direct=true,color= black, lw =1pt](phi)(x)
\Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)
\Edge[Direct=true,color= black,lw =1pt](sigma)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
\end{tikzpicture}
  %\vspace{-0.2cm}
    \caption{Gaussian Process model} \label{fig:graph_color}
    %\vspace{-0.15cm}
\end{figure}
\fi

Consider a set of $K$ time-dependent states denoted as $\textbf{x}(t)= [x_1(t),\dots,x_K(t)]^T$.
The evolution of each of these $K$ state over time is defined by a set of $K$ time-dependent arbitrary differential equations denoted as follows:
% %\vspace{-0.4cm}
\begin{equation}\label{eq:def_ode}
    \displaystyle \dot{x}_i(t) = \frac{d{x}_i(t)}{dt} =  \text{f}_i(x(t),\theta,t)   \quad \forall \quad i \in \{ 1, \dots, K\}
\end{equation}

where the functional form of $\text{f}_i$ is known (for eg. SEIR model). Noisy observations (i.e. the time-series data) of  each of the $K$ states (denoted $\textbf{y}(t) = [ y_1(t),\dots,y_K(t)  ]^T$) at $N$ different time points where $t_1 < \dots < t_N $ are available, i.e. 
%for any $t \in \{t_1 ,\dots,t_N\}$ we have
%$ {y}_i(t_j) = {x}_i(t_j) + \epsilon_i(t_j) \;\; \forall  \;\; i \in \{ i, \dots, K\} , \; \text{where} \;\;\epsilon_i(t) \sim \mathcal{N}(0,\sigma^2_i)$.
\begin{equation*}
\begin{rcases}
\begin{matrix}
    y_1(t)  =  x_1(t)  +  \epsilon_1(t) \\ 
    \vdots   \\ 
    y_K(t)  =  x_K(t) +  \epsilon_K(t) \\ 
\end{matrix} 
\end{rcases} \;, 
\begin{aligned}
  &\text{ where } \epsilon_i(t) \sim \mathcal{N}(0,\sigma^2_i). \\  
  & \;\; \forall \;\; t \in  \{t_1 ,\dots,t_N\}
\end{aligned}  
\end{equation*}
Let $\bm{\epsilon}(t) = [ \epsilon_1(t),\dots,\epsilon_K(t)  ]^T$, then in vector notation we have $\textbf{y}(t) = \textbf{x}(t) + \bm{\epsilon}(t) $.
As there are  $N$ observations for each of the $K$ states, for a clear exposition we introduce matrices of size $K \times N$ as follows: $\textbf{X}  = [ \textbf{x}(t_1), \dots, \textbf{x}(t_N) ]$ and $\textbf{Y}  = [ \textbf{y}(t_1), \dots, \textbf{y}(t_N) ]$.
We can then write :
\begin{alignat}{10}
\displaystyle P(\textbf{Y}| \textbf{X}, \sigma) &= \prod_{k} \prod_{t} P(y_k(t)| x_k(t),\sigma) =\prod_{k} \prod_{t} \mathcal{N}(y_k(t)| x_k(t),\sigma^2) \label{eq:y_given_x_sigma}
\end{alignat}
 
%The high computational cost associated with explicit numerical integration 
\cite{calderhead} proposed placing a Gaussian process prior on $\textbf{x}_k$. 
Let $\bm{\mu}_k$ and $\bm{\phi}_k$ be the hyper-parameters of this Gaussian process, we can then write:
%\vspace{-0.2cm}
\begin{equation}\label{eq:gp}
p(\textbf{x}_k|\bm{\mu}_k,\bm{\phi}_k) = \mathcal{N}(\textbf{x}_k | \bm{\mu}_k, \textbf{C}_{\phi_{k}})
%\vspace{-0.2cm}
\end{equation}

In \eqref{eq:gp}, $\textbf{C}_{\phi_{k}}$, denotes the Kernel (or the covariance) matrix for a predefined kernel function with hyper-parameters $\bm{\phi}_k$. 
As differentiation is a linear operator therefore the derivative of a Gaussian process is also a Gaussian process (see ch-9 in \cite{rasmussen}  and \cite{solak}). Therefore a Gaussian process is closed under differentiation and the joint distribution of the state variables $\textbf{x}_k$ and their derivatives $\dot{\textbf{x}}_k$ is a multi-variate Gaussian distribution as follows:
%\vspace{-0.25cm}
\begin{equation}\label{eq:joint_x_xdot}
\begin{bmatrix}
\textbf{x}_k \\
\dot{\textbf{x}}_k
\end{bmatrix} \sim \mathcal{N}\bigg(
\begin{bmatrix}
\bm{\mu}_k \\
\bm{0}
\end{bmatrix} ,
\begin{bmatrix}
 \textbf{C}_{\phi_{k}} , '\textbf{C}_{\phi_{k}} \\
 \textbf{C}'_{\phi_{k}}, \textbf{C}''_{\phi_{k}}
\end{bmatrix}
\bigg)
\end{equation}

where $\textbf{C}_{\phi_{k}}$ and $\textbf{C}''_{\phi_{k}}$ are the kernel matrices for the state $\textbf{x}_k$ and its derivative $\dot{\textbf{x}}_k$ respectively, while  $'\textbf{C}_{\phi_{k}} \text{ and } \textbf{C}'_{\phi_{k}}$ are the cross-covariance kernel matrices between the states and their derivatives. The functional form of the entries of $\textbf{C}_{\phi_{k}}, \textbf{C}''_{\phi_{k}}, 
'\textbf{C}_{\phi_{k}} \text{ and } \textbf{C}'_{\phi_{k}} $ are provided in SI. Importantly, this implies that using the Gaussian process defined on the state variables $\textbf{x}_k$, we can also make predictions about their derivatives  $\dot{\textbf{x}}_k$. 
%Corresponding graphical models are shown in fig. \ref{fig:ode_gp_model}. 
From \eqref{eq:joint_x_xdot}, we can compute the conditional distribution of the state derivatives as:
%\vspace{-0.3cm}
\begin{equation}\label{eq:graph_2}
p(\dot{\textbf{x}}_k | \textbf{x}_k, \bm{\mu}_k, \bm{\phi}_k)  = \mathcal{N}(\dot{\textbf{x}}_k |\textbf{m}_k,\textbf{A}_k )
\end{equation}
%$$ p(\dot{\textbf{x}}_k | \textbf{x}, \bm{\mu}_k, \bm{\phi}_k)  = \mathcal{N}(\dot{\textbf{x}}_k |\textbf{m}_k,\textbf{A}_k ), \quad \text{ where} $$
where $\textbf{m}_k = '\textbf{C}_{\phi_{k}}{\textbf{C}_{\phi_{k}}}^{-1} (\textbf{x}_k - \bm{\mu}_k ); \;\textbf{A}_k = \textbf{C}''_{\phi_{k}} - '\textbf{C}_{\phi_{k}}{\textbf{C}_{\phi_{k}}}^{-1}\textbf{C}'_{\phi_{k}}$. Note that $p(\dot{\textbf{x}}_k | \textbf{x}_k, \bm{\mu}_k, \bm{\phi}_k)$ corresponds to the second, i.e. GP part of the graphical model in fig. \ref{fig:ode_gp_model}.

Using the functional form of the ODE system in \eqref{eq:def_ode} and with state specific Gaussian additive noise $\gamma_k$, we can write
\begin{equation}\label{eq:graph_1}
    p(\dot{\textbf{x}}_k| \textbf{X},\bm{\theta},\gamma_k) = \mathcal{N}( \dot{\textbf{x}}_k |\textbf{f}_k(\textbf{X}, \bm{\theta}) , \gamma_k\textbf{I})
\end{equation}

where $\textbf{f}_k(\textbf{X}, \bm{\theta}) = [ \text{f}_k(\text{x}(t_1), \bm{\theta} ),\dots,\text{f}_k(\text{x}(t_N), \bm{\theta} )   ]^T$.
%This key insight was the major motivation behind the "Gradient matching" approach of  \cite{dondelinger}. 
Note that \eqref{eq:graph_1} corresponds to the ODE part of the graphical model in the fig. \ref{fig:ode_gp_model}.

\begin{figure}[h!]
\vspace{-0.2cm}
\begin{minipage}{0.35\linewidth}
    \SetVertexStyle[TextFont= \Large]
    %\begin{figure}[ht]
    %\vspace{-0.0cm}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tikzpicture}
    
    \begin{pgfonlayer}{background}
    %\filldraw[color = red,rounded corners]
    % (-0.6,-0.5)--(-0.6,2.5)--(3,-0.5)--cycle;
     \draw[color =red, style= dashed, rounded corners=0.2cm] (-0.75, -0.6) rectangle (3.3, 2.1) {};
     \draw[color =blue,style= dashed, rounded corners=0.2cm] (3.5, -0.6) rectangle (7.5, 2.1) {};
    \end{pgfonlayer}
    
    \Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=1.3, y=0 ]{x_dot_ode}
    \Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=-0.2,   y=0 ]{theta}
    \Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=2.8,   y=0]{x_ode}
    \Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=1.3, y=1.5 ]{gamma}
    \Edge[Direct=true,color= black, lw =1pt](theta)(x_dot_ode)
    \Edge[Direct=true,color= black,lw =1pt](gamma)(x_dot_ode)
    \Edge[Direct=true,color= black,lw =1pt](x_ode)(x_dot_ode)
    \node at (1.3,-1) { {\Large ODE model}};
    
    \Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=4, y=1.5 ]{x_dot}
    \Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=5.5, y=1.5]{x}
    \Vertex[ size= 0.8,opacity =0, label = $\textbf{y}$,             x=7, y=1.5 ]{y}
    \Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=5.5, y=0 ]{phi}
    \Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=7, y=0 ]{sigma}
    \Edge[Direct=true,color= black, lw =1pt](phi)(x)
    \Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)
    \Edge[Direct=true,color= black,lw =1pt](sigma)(y)
    \Edge[Direct=true,color= black,lw =1pt](x)(y)
    \Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
    \node at (5.5,-1) { {\Large GP model}};
    
    \Edge[Direct=false,style =dashed, color= black, lw =1pt](x_dot_ode)(x_dot)
    \Edge[Direct=false,style=dashed, color= black,lw =1pt](x_ode)(x)
    
    \end{tikzpicture}
    }
      %\vspace{-0.25cm}
        %\caption{ODE model and Gaussian Process model} \label{fig:ode_gp_model}
        \caption{ODE model and GP model} \label{fig:ode_gp_model}
        %%\vspace{-0.4cm}
    %\end{figure}    
\end{minipage}\hfill
\begin{minipage}{0.58\linewidth}
%\begin{small}
%%\vspace*{-0.4cm}
\SetVertexStyle[TextFont= \Large]
%\begin{figure}[ht]
%%\vspace{-0.25cm}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=5, y=1.5 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=5, y=0 ]{gamma}
\Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=3.5,  y=1.5 ]{theta}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=6.5, y=1.5]{x}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{y}$,         x=8, y=1.5 ]{y}
\Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=6.5, y=0 ]{phi}
\Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=8, y=0 ]{sigma}

\Edge[Direct=true,color= black, lw =1pt](phi)(x)
\Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)

\Edge[Direct=true,color= black,lw =1pt](gamma)(x_dot)
\Edge[Direct=true,color= black,lw =1pt](theta)(x_dot)

\Edge[Direct=true,color= black,lw =1pt](sigma)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)

\draw [-> , line width=0.2em ](9.0,1) -- (10.5,1);
\node[text width=1cm] at (9.4,1.6) {{\Large after}};
\node[text width=3cm] at (10.4,0.3) { {\Large marginalization}};
\node[text width=1cm] at (9.4,-0.3) {{\Large of $\dot{\textbf{x}}$}};

%\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,  x=4, y=1.5 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=13.5, y=0 ]{gamma1}
\Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=12,  y=1.5 ]{theta1}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=15, y=1.5]{x1}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{y}$,         x=16.5, y=1.5 ]{y1}
\Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=15, y=0 ]{phi1}
\Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=16.5, y=0 ]{sigma1}

\Edge[Direct=true,color= black, lw =1pt](phi1)(x1)
%\Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)

%\Edge[Direct=true,color= black,lw =1pt](gamma)(x_dot)
%\Edge[Direct=true,color= black,lw =1pt](theta)(x_dot)

\Edge[Direct=true,color= black,lw =1pt](sigma1)(y1)
\Edge[Direct=true,color= black,lw =1pt](x1)(y1)
%\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
%\node at (5.5,-1) { GP model};
\end{tikzpicture}
}
 %\vspace{-0.2cm}
    \caption{Graphical model using PoE (on left) and  the model 
 (on right ) after marginalization of $\dot{\textbf{x}}$. }  \label{fig:poe_marginal}
 %\vspace{-0.5cm}
%\end{figure}
%\end{small}
\end{minipage}
\vspace{-0.2cm}
\end{figure}

The two models $p(\dot{\textbf{x}}_k | \textbf{x}_k, \bm{\mu}_k, \bm{\phi}_k)$ in \eqref{eq:graph_2} and $p(\dot{\textbf{x}}| \textbf{X},\bm{\theta},\gamma_k)$ in \eqref{eq:graph_1} are next combined using a product of experts (PoE) approach \cite{prod_of_exp}.
The use of PoE to combine the two models (see fig. \ref{fig:poe_marginal}) was originally proposed by \cite{calderhead} and also used by \cite{dondelinger}. 
In the PoE approach the two models are combined to get the distribution of $p(\dot{\textbf{x}}_k| \textbf{X}, \bm{\theta}, \bm{\phi}, \gamma_k)$ as follows:
\begin{alignat}{10}
p(\dot{\textbf{x}}_k| \textbf{X}, \bm{\theta}, \bm{\phi},& \gamma_k ) \propto p(\dot{\textbf{x}}_k | \textbf{x}_k, \bm{\mu}_k, \bm{\phi}_k)p(\dot{\textbf{x}}| \textbf{X}, \bm{\theta},\gamma_k) \mathcal{N}(\dot{\textbf{x}}_k |\textbf{m}_k,\textbf{A}_k )\mathcal{N}(\dot{\textbf{x}}_k | \textbf{f}_k(\textbf{X}, \bm{\theta}) , \gamma_k\textbf{I}) \label{eq:poe}
\end{alignat}

After marginalization over $\dot{\textbf{x}}_k$ , \cite{dondelinger} were able to write the joint-probability for the whole system as follows (see SI for mathematical details): 
\begin{alignat}{10}
&p(\textbf{Y}, \textbf{X}, \bm{\theta}, \bm{\phi},\bm{\gamma}, \bm{\sigma}) \propto p(\textbf{Y} | \textbf{X}, \bm{\sigma}) p(\textbf{X}| \bm{\theta}, \bm{\phi},\bm{\gamma})p(\bm{\theta}) p(\bm{\phi}) p(\bm{\gamma}) p(\bm{\sigma}) \label{eq:system_joint}
\end{alignat}

Finally, \cite{dondelinger} developed a Metropolis-Hastings based sampling scheme to sample $\textbf{X}, \bm{\theta}, \bm{\phi},\bm{\gamma}, \bm{\sigma}$ directly from the posterior distribution $p(\textbf{X}, \bm{\theta}, \bm{\phi},\bm{\gamma}, \bm{\sigma}| \textbf{Y}) \propto p(\textbf{Y}, \textbf{X}, \bm{\theta}, \bm{\phi},\bm{\gamma}, \bm{\sigma})$.
In summary, the use of PoE heuristics in literature is common. Both \cite{calderhead} and \cite{dondelinger} using PoE  were able to get good estimates for $\bm{\theta}$ using MCMC sampling procedures.

\iffalse

\SetVertexStyle[TextFont= \Large]
\begin{figure}[ht]
%%\vspace{-0.25cm}
\centering
\resizebox{0.5\linewidth}{!}{%
\begin{tikzpicture}
%\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=4, y=1.5 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=4, y=0 ]{gamma}
\Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=2.5,  y=1.5 ]{theta}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=5.5, y=1.5]{x}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{y}$,             x=7, y=1.5 ]{y}
\Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=5.5, y=0 ]{phi}
\Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=7, y=0 ]{sigma}

\Edge[Direct=true,color= black, lw =1pt](phi)(x)
%\Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)

%\Edge[Direct=true,color= black,lw =1pt](gamma)(x_dot)
%\Edge[Direct=true,color= black,lw =1pt](theta)(x_dot)

\Edge[Direct=true,color= black,lw =1pt](sigma)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(y)
%\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
%\node at (5.5,-1) { GP model};
\end{tikzpicture}
}
  %\vspace{-0.2cm}
    \caption{Graphical model resulting after marginalization of $\dot{\textbf{x}}$. }  \label{fig:poe_marginal}
 %\vspace{-0.5cm}
\end{figure}
\fi

However, \cite{fgpgm} noted that after the marginalization of $\dot{\textbf{X}}$,
%in \eqref{eq:margianl_x_dot}
the PoE graphical model results in the graphical model shown in \ref{fig:poe_marginal}. In this graphical model there is no link between the parameters $\bm{\theta}$ and the observations $\textbf{y}$, thus defeating the whole purpose of combining the ODE model and GP model (in figure \ref{fig:ode_gp_model}) using PoE. 
%\cite{fgpgm} also showed this discrepancy mathematically, using the derivations from the \cite{calderhead}.
To fix this discrepancy, an alternative graphical model shown in figure \ref{fig:fgpgm_model}  was proposed by \cite{fgpgm}.

\SetVertexStyle[TextFont= \Large]
\begin{wrapfigure}{r}{0.25\linewidth}
%\begin{figure}[ht]
\vspace{-0.55cm}
\centering
  \captionsetup{singlelinecheck=on, margin={0.0cm, 0.0cm}, justification=justified, format=plain}
\resizebox{0.9\linewidth}{!}{%
\begin{tikzpicture}
\Vertex[ size= 0.8,opacity =0, label = $\dot{\textbf{x}}$,   x=4, y=1.5 ]{x_dot}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{x}$,         x=5.5, y=1.5]{x}
\Vertex[ size= 0.8,opacity =0, label = $\textbf{y}$,             x=7, y=1.5 ]{y}
\Vertex[ size= 0.8,opacity =0, label = $\phi$,               x=5.5, y=0 ]{phi}
\Vertex[ size= 0.8,opacity =0, label = $\sigma$,             x=7, y=0 ]{sigma}
\Vertex[ size= 0.8,opacity =0, label = $\text{F}_1$,   x=5.5, y=3 ]{F_1}
\Vertex[ size= 0.8,opacity =0, label = $\text{F}_2$,   x=4, y=3 ]{F_2}
\Vertex[ size= 0.8,opacity =0, label = $\gamma$,             x=2.5, y=3 ]{gamma}
\Vertex[ size= 0.8,opacity =0, label = $\bm{\theta}$,        x=7,  y=3 ]{theta}

\Edge[Direct=true,color= black, lw =1pt](phi)(x)
\Edge[Direct=true,color= black,lw =1pt](phi)(x_dot)
\Edge[Direct=false,color= black,lw =1pt](F_1)(F_2)
\Edge[Direct=true,color= black,lw =1pt](gamma)(F_2)
\Edge[Direct=true,color= black,lw =1pt](theta)(F_1)
\Edge[Direct=true,color= black,lw =1pt](x_dot)(F_2)
\Edge[Direct=true,color= black,lw =1pt](x)(F_1)
\Edge[Direct=true,color= black,lw =1pt](sigma)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(y)
\Edge[Direct=true,color= black,lw =1pt](x)(x_dot)
%\node at (5.5,-1) { GP model};
\end{tikzpicture}
}
  %\vspace{-0.4cm}
  \begin{small}
    \caption{Corrected model.}%  proposed by \cite{fgpgm}} 
    %\caption{\cite{fgpgm}}
    \label{fig:fgpgm_model}
  \end{small}  
    %\vspace{-0.3cm}
%\end{figure}
\end{wrapfigure}

In the new graphical model two new random variables $\textbf{F}_1$ and $\textbf{F}_2$ are introduced, through which the two models (i.e the GP model and the ODE model) are combined as shown in fig. \ref{fig:fgpgm_model}.
For given values of $\textbf{x}$ and $\bm{\theta}$, $\textbf{F}_1$ in fig. \ref{fig:fgpgm_model}, represents the deterministic output of the ODEs, i.e. $\textbf{F}_1= \textbf{f}(\bm{\theta}, \textbf{x})$. The value of $p(\textbf{F}_1| \bm{\theta}, \textbf{x})$ can be written using the Dirac-delta function (denoted $\delta(\cdot)$) as following:
\begin{equation}
p(\textbf{F}_1| \bm{\theta}, \textbf{x}) = \delta(\textbf{F}_1- \textbf{f}(\bm{\theta}, \textbf{x})) 
%\vspace{-0.25cm}
\end{equation}

Under the assumption that the GP model would be able to capture both, the true states and their derivatives perfectly, then it would imply that $\textbf{F}_1$ is same as $\dot{\textbf{x}}$, i.e.  $\textbf{F}_1 = \dot{\textbf{x}}$. But clearly this assumption is unlikely to hold, therefore to account for any possible mismatch and small error in  the GP states and GP derivatives, this condition is relaxed so that:
%\vspace{-0.25cm}
\begin{equation}\label{eq:equality_f1_f2}
 \textbf{F}_1 = \dot{\textbf{x}} + \epsilon \eqqcolon \textbf{F}_2, \quad \text{ where } \quad \epsilon \sim \mathcal{N}(\bm{0}, \gamma \textbf{I})  
 %\vspace{-0.25cm}
\end{equation}


The above argument regarding the the error in the states and derivatives of the GP model is captured in the graphical model (fig. \ref{fig:fgpgm_model}) through the use of the random variable $\textbf{F}_2$. From a given state-derivative $\dot{\textbf{x}}$ obtained from the GP model, $\textbf{F}_2$ is obtained after addition of Gaussian noise with standard deviation $\gamma$. The probability density of $\textbf{F}_2$ can then be written as    
%\vspace{-0.2cm}
\begin{equation}
p(\textbf{F}_2|\dot{\textbf{x}}, \gamma) = \mathcal{N}(\textbf{F}_2 | \dot{\textbf{x}}, \gamma \textbf{I})) 
\end{equation}
%%\vspace{-0.2cm}
Note that the equality constraint in \eqref{eq:equality_f1_f2} is encoded in the graphical model using an un-directed edge between $\textbf{F}_1$ and $\textbf{F}_2$. For the purpose of  inference, this equality constraint is incorporated in the joint density via the Dirac-delta function, i.e. $\delta(\textbf{F}_1 - \textbf{F}_2)$. The joint-density of the whole graphical model (fig. \ref{fig:fgpgm_model}), considering a single state (for notational simplicity) is given as:
%\vspace{-0.2cm}
\begin{alignat}{10}
p(\textbf{x}, \dot{\textbf{x}}, \textbf{y}, \textbf{F}_1,\textbf{F}_2, \bm{\theta}| \phi, \sigma, \gamma ) = & p(\bm{\theta}) p(\textbf{x}|\phi) p(\dot{\textbf{x}} | \textbf{x},\phi) p(\textbf{y}| \textbf{x}, \sigma) p(\textbf{F}_1| \bm{\theta}, \textbf{x}) & p(\textbf{F}_2| \dot{\textbf{x}}, \gamma \textbf{I})\delta( \textbf{F}_1-\textbf{F}_2)
\end{alignat}
%\vspace{-0.7cm}


Finally, the marginal distribution of $\textbf{x},\bm{\theta}$ takes the following form:
%\vspace{-0.2cm}
\begin{alignat}{10}
&p(\textbf{x},\bm{\theta} |\textbf{y}, \bm{\phi}, \sigma, \gamma ) =  p(\bm{\theta}) \times \mathcal{N}(\textbf{x}| \bm{\mu}, \textbf{C}_{\phi}) \times \mathcal{N}(\textbf{y}|\textbf{x}, \sigma^2 \textbf{I} )\times \mathcal{N}(\textbf{f}(\textbf{x}, \bm{\theta})|\textbf{m}, \textbf{A} + \gamma \textbf{I} ) \label{eq:fgpgm}
\end{alignat}

%Using \eqref{eq:fgpgm}, the distribution over $\theta$ can be obtained with the . \\

%%\vspace{-0.25cm}

